Galaxy mergers in EAGLE do not induce a significant amount of black hole growth yet do increase the rate of luminous AGN

We investigate the connection between galaxy--galaxy mergers and enhanced black hole (BH) growth using the cosmological hydrodynamical EAGLE simulation. We do this via three methods of analysis, investigating: the merger fraction of AGN, the AGN fraction of merging systems and the AGN fraction of galaxies with close companions. In each case, we find an increased abundance of AGN within merging systems relative to control samples of inactive or isolated galaxies (by up to a factor of $\approx 3$ depending on the analysis method used), confirming that mergers are enhancing BH accretion rates for at least a subset of the galaxy population. The greatest excess of AGN triggered via a merger are found in lower mass ($M_* \sim 10^{10}$~\Msol) gas rich ($f_{\mathrm{gas}} > 0.2$) central galaxies with lower mass BHs ($M_{\mathrm{BH}} \sim 10^{7}$~\Msol) at lower redshifts ($z<1$). We find no enhancement of AGN triggered via mergers in more massive galaxies ($M_* \gtrsim 10^{11}$~\Msol). The enhancement of AGN is not uniform throughout the phases of a merger, and instead peaks within the early \emph{remnants} of merging systems (typically lagging $\approx 300$~Myr post-coalescence of the two galaxies at $z=0.5$). We argue that neither major ($M_{\mathrm{*,1}} / M_{\mathrm{*,2}} \geq \frac{1}{4}$) nor minor mergers ($\frac{1}{10} < M_{\mathrm{*,1}} / M_{\mathrm{*,2}} < \frac{1}{4}$) are statistically relevant for enhancing BH masses globally. Whilst at all redshifts the galaxies experiencing a merger have accretion rates that are on average 2--3 times that of isolated galaxies, the majority of mass that is accreted onto BHs occurs outside the periods of a merger. We compute that on average no more than 15\% of a BHs final day mass comes from the enhanced accretion rates triggered via a merger

==> ToAdd.tex <==
\begin{figure} \includegraphics[width=\columnwidth]{plots/close_pairs_z_0_1.pdf}

\caption{\textit{Top}: the AGN fraction as a function of pair separation for galaxies in the redshift range $0 < z < 1$ with stellar masses $M_{\mathrm{*,1}} \geq 10^{10}$ \Msol that have a close companion with stellar mass $M_{\mathrm{*,2}}$ satisfying $\frac{1}{4} \leq M_{\mathrm{*,1}} / M_{\mathrm{*,2}} \leq 4$. For comparison, the AGN fraction for a mass-matched sample of isolated galaxies (no companion within 100 pkpc) is also shown. The shaded regions are the Poison uncertainty. \textit{Bottom}: the difference in the AGN fraction between the galaxies with close companions and the mass-matched control sample of isolated galaxies. The galaxies with companions $\gtrsim 80$ pkpc have AGN fractions consistent with those of isolated galaxies. With decreasing pair separation, the excess in the AGN fraction above the control sample increases to up to a factor of $\approx 2$.1}

\label{fig:close_pairs_z_0_1}
\end{figure}

\begin{figure} \includegraphics[width=\columnwidth]{plots/close_pairs_z_1_2.pdf}

\caption{The same as \cref{fig:close_pairs_z_0_1} but for $1 < z < 2$.}

\label{fig:close_pairs_z_1_2}
\end{figure}

\begin{figure} \includegraphics[width=\columnwidth]{plots/close_pairs_z_2_5.pdf}

\caption{The same as \cref{fig:close_pairs_z_0_1} but for $2 < z < 5$.}

\label{fig:close_pairs_z_0_1}
\end{figure}




\begin{figure*} \includegraphics[width=\textwidth]{plots/individual_history.pdf}

\caption{Need to think about this figure a bit more. But its to demostrate how the timescales compare against the morphology of the galaxy.}

\label{fig:individual_history}
\end{figure*}






\subsection{The AGN fraction of close pairs}
\label{sect:close_pairs}

\begin{figure} \includegraphics[width=\columnwidth]{plots/close_pairs_z_0_1.pdf}

\caption{\textit{Top}: the AGN fraction as a function of pair separation for galaxies in the redshift range $0 < z < 1$ with stellar masses $M_{\mathrm{*,1}} \geq 10^{10}$ \Msol that have a close companion with stellar mass $M_{\mathrm{*,2}}$ satisfying $\frac{1}{4} \leq M_{\mathrm{*,1}} / M_{\mathrm{*,2}} \leq 4$. For comparison, the AGN fraction for a mass-matched sample of isolated galaxies (no companion within 100 pkpc) is also shown. The shaded regions are the Poison uncertainty. \textit{Bottom}: the difference in the AGN fraction between the galaxies with close companions and the mass-matched control sample of isolated galaxies. The galaxies with companions $\gtrsim 80$ pkpc have AGN fractions consistent with those of isolated galaxies. With decreasing pair separation, the excess in the AGN fraction above the control sample increases to up to a factor of $\approx 2$.1}

\label{fig:close_pairs_z_0_1}
\end{figure}

\begin{figure} \includegraphics[width=\columnwidth]{plots/close_pairs_z_1_2.pdf}

\caption{The same as \cref{fig:close_pairs_z_0_1} but for $1 < z < 2$.}

\label{fig:close_pairs_z_1_2}
\end{figure}

\begin{figure} \includegraphics[width=\columnwidth]{plots/close_pairs_z_2_5.pdf}

\caption{The same as \cref{fig:close_pairs_z_0_1} but for $2 < z < 5$.}

\label{fig:close_pairs_z_0_1}
\end{figure}

We note, that as was the case in \cref{sect:merger_fraction}, the majority of the excess in the AGN fraction comes from the BHs in the remnants of merging systems and not those in the interacting phase. Also, the resulting excess is again largely insensitive to the way in which the control sample is formed: the values of the excess are similar if the isolated control galaxies are paired only on the stellar mass, or on all of the stellar, total gas and BH masses. If the SFR is also considered for pairing the control galaxies, the excess drops, as was also the case for the merger fraction of AGN (see \cref{sect:choosing_control_sample}).  
\begin{figure} \includegraphics[width=\columnwidth]{plots/effect_of_control_edd.pdf}

\caption{The excess in the major merger fraction between the AGN and their inactive control galaxies as a function of the Eddington rate (see \cref{fig:major_merger_fraction}). Each panel shows how the trends in the excess change as the criteria of the control sample is redefined. Matching the control galaxies on the stellar mass alone yields very similar results to matching on the stellar, gas and BH masses. If the SFR is also included in the pairing criteria, the excess dramatically drops. This is because star formation is also enhanced during the merger process.}

\label{fig:effect_of_control}
\end{figure}


